Automated Classification of Overfitting Patches with Statically Extracted Code Features

Automatic program repair (APR) aims to reduce the cost of manually fixing software defects. However, APR suffers from generating a multitude of overfitting patches, those patches that fail to correctly repair the defect beyond making the tests pass. This paper presents a novel overfitting patch detection system called ODS to assess the correctness of APR patches. ODS first statically compares a patched program and a buggy program in order to extract code features at the abstract syntax tree (AST) level. Then, ODS uses supervised learning with the captured code features and patch correctness labels to automatically learn a probabilistic model. The learned ODS model can then finally be applied to classify new and unseen program repair patches. We conduct a large-scale experiment to evaluate the effectiveness of ODS on patch correctness classification based on 10,302 patches from Defects4J, Bugs.jar and Bears benchmarks. The empirical evaluation shows that ODS is able to correctly classify 71.9% of program repair patches from 26 projects, which improves the state-of-the-art. ODS is applicable in practice and can be employed as a post-processing procedure to classify the patches generated by different APR systems.

==> listings/Time19-false-positive.tex <==
\begin{listing}[h!]
\caption{False positive case of Time19 from PatchHDRepair10 }
\label{lst:fpmath85}
\begin{lstlisting}
-   } else if (offsetLocal > 0) {
+   } else if (offsetLocal >= 0) {
\end{lstlisting}
\end{listing}

==> listings/math85-false-positives.tex <==
\begin{listing}[th!]

\begin{lstlisting}
 - if (fa * fb >= 0.0 ){
 + if (fa * fb >= 0.0 &&!(fa * fb==0.0)){
 // if (fa * fb > 0.0){ human-written patch
\end{lstlisting}
\caption{False positive case of Math-85 from Patch204 }
\label{lst:fpmath85}
\end{listing}

==> tables/False-positives.tex <==
\begin{table*}[t!]
\footnotesize
\renewcommand{\arraystretch}{2}
\centering
\begin{tabularx}{0.85\textwidth}{@{}X|XXX|XXX|XXX@{}}
\hline

\end{tabularx}
Project & 12
FasterXML-jackson & 13 & 11 & 2 & 15.4\% \\


\caption{False positives}	
\label{tab:falsepositives}
\end{table*}

==> tables/ODSDataSet.tex <==
\begin{table}
\footnotesize
\centering
\renewcommand{\arraystretch}{1.4}
\begin{tabularx}{0.47\textwidth}{@{}Xrrr@{}}
\hline
Benchmark &\# correct patches &\# overfitting patches& \# total\\
\hline
Defects4J & 807 & 5493 & 6300 \\
Bugs.jar & 986 & 2275 & 3261 \\
Bears & 210 & 531 & 741 \\
\hline
Total& 2003 & 8299 & \textbf{10302}  \\
\hline
\end{tabularx}
\caption{ODS training dataset}	
\label{tab:ODSTrainingData}
\end{table}

==> tables/RQ1WithInBenResult.tex <==
\begin{table*}[t!]
\footnotesize
\renewcommand{\arraystretch}{3}
\centering
\begin{tabular}{@{}l|rrr|rrr|rrr|rrr@{}}
\hline


\multirow{2}{*}{ \diagbox{Validation}{Training} } & \multicolumn{3}{c|}{Random  (Baseline) } &\multicolumn{3}{c|}{5-fold Cross Validation } & \multicolumn{3}{c|}{Bugs.jar+Bears}& \multicolumn{3}{c}{Defects4J }\\

\cline{2-13}


  &   P & R &F1  &   P & R& F1  &P  & R& F1 &P  & R& F1 \\
\hline 
\multirow{1}{*}{Defects4J}  & 86.5\% & 48.5\% &  62.1\% & 94.3\% & 80.3 \%& 86.7 \%& 90.6 \%& 79.6\% & 84.7\%\\



\hline
\multirow{1}{*}{Bugs.jar} & 68.4\% & 49.5\% & 57.4\%& 92.2 \%& 91.0 \%& 91.6 \%& && & 82.5 \%& 72.5\% & 77.2 \%  \\


\hline
\multirow{1}{*}{Bears} & 70.9\% & 48.6\% & 57.7 \% & 94.2\% & 94.8 \%& 94.5\% &&&& 86.2 \%& 77.2\% & 81.4\%\\

\hline
\multirow{1}{*}{Average } &75.3 \% & 48.9\% & 59.1\% & 93.6\% & 88.7\% & 91.0 \%&  \multicolumn{2}{c}{P: 86.4\%} & \multicolumn{2}{c}{R :76.4\%} & \multicolumn{2}{c}{F1 : 81.1 \%}      \\


\hline
\end{tabular}
\caption{ Precision (P), recall (R) and F1 scores of ODS using within benchmark (5-fold cross validation) and inter-benchmark training and validation.}	
\label{tab:rq1}
\end{table*}

% defects4j -> bears: use smote and map

==> tables/RQ2.tex <==
\begin{table*}[t!]
\scriptsize
\renewcommand{\arraystretch}{3}
\begin{tabular}{ccccc}
\hline
 Project & C & O & \\
 \hline
 
 Lang & 102 & 49 \\

 Chart & 98 & 55  \\

 Math & 245 & 103  \\

Time & 2 & 4 \\
\hline
Total &654&248 
& \\
\hline


\end{tabular}
\caption{Comparison between ODS and integration of existing patch assessment technique on 902 patches (All - P = all training patches minus patches from project P, O=Overfitting patches, C=Correct patches )
}	
\label{tab:rq2}
\end{table*}


